Algorithmic Regularization in Learning Deep Homogeneous Models: Layers are Automatically Balanced

We study the implicit regularization imposed by gradient descent for learning multi-layer homogeneous functions including feed-forward fully connected and convolutional deep neural networks with linear, ReLU or Leaky ReLU activation. We rigorously prove that gradient flow (i.e. gradient descent with infinitesimal step size) effectively enforces the differences between squared norms across different layers to remain invariant without any explicit regularization. This result implies that if the weights are initially small, gradient flow automatically balances the magnitudes of all layers. Using a discretization argument, we analyze gradient descent with positive step size for the non-convex low-rank asymmetric matrix factorization problem without any regularization. Inspired by our findings for gradient flow, we prove that gradient descent with step sizes $\eta_t = O\left(t^{-\left( \frac12+\delta\right)} \right)$ ($0<\delta\le\frac12$) automatically balances two low-rank factors and converges to a bounded global optimum. Furthermore, for rank-$1$ asymmetric matrix factorization we give a finer analysis showing gradient descent with constant step size converges to the global minimum at a globally linear rate. We believe that the idea of examining the invariance imposed by first order algorithms in learning homogeneous models could serve as a fundamental building block for studying optimization for learning deep models.

==> pre.tex <==






%For a matrix $\mat{A}$, we use $\lambda_{\max}\left(\mat{A}\right)$ to denote its eigenvalue and $\lambda_{\min}\left(\mat{A}\right)$ its smallest singular value.
%Let $O(\cdot)$, $\Omega\left(\cdot\right)$ and $\Theta\left(\cdot\right)$ denote standard Big-O, Big-Omega and Big-Theta notations, only hiding absolute constants.
%
%In this paper, we characterize the landscape of  over-parameterized neural networks.
%More specifically we study the properties of critical points of empirical loss.
%Here for a loss function $L\left(\mat{W}\right)$, a critical point $\mat{W}^*$ satifies $\nabla L\left(\mat{W}^*\right) = 0$.
%A critical point can be a local minimum or a saddle point.\footnote{We do not differentiate between saddle points and local maxima in this paper.}
%If $\mat{W}^*$ is a local minimum, then there is a neighborhood $O$ around $\mat{W}^*$ such that $L\left(\mat{W}^*\right) \le L\left(\mat{W}\right)$ for all $\mat{W} \in O$.
%If $\mat{W}^*$ is a saddle point, then for all neighborhood $O$ around $\mat{W}^*$, there is a $\mat{W} \in O$ such that $L\left(\mat{W}\right) < L\left(\mat{W}^*\right)$.
%
%Ideally, we would like a loss function satisfy the following two geometric properties.
%\begin{property}[All local minima are global]\label{prop:local_global}
%	If $\mat{W}^*$ is a local minimum of $L\left(\cdot\right)$ it is also the global minimum, i.e., $\mat{W}^* \in \argmin_{\mat{W}}L\left(\mat{W}\right)$.
%\end{property}
%\begin{property}[All saddles are strict]\label{prop:saddle_strict}
%	At a saddle point $\mat{W}_s$, there is a direction $\mat{U}\in\mathbb{R}^{k \times d}$ such that \begin{align*}
%	\vectorize{\mat{U}}^\top \nabla^2L\left(\mat{W}_s\right) \vectorize{\mat{U}} < 0.
%	\end{align*}
%	% \jason{Did you actually prove this property?? Is this easy to show? A bit concerned that this might be hard to show, I ahve't tried to compute the hessians at all.}
%	% \simon{We prove that if a $\mat{W}$ satisfy gradient = 0 and hessian psd, it must be a global optimal.
%	% 	This implies these two properties simultaneously.
%	% 	}
%\end{property}
%If a loss function $L\left(\cdot\right)$ satisfies Property~\ref{prop:local_global} and Property~\ref{prop:saddle_strict}, recent algorithmic advances in non-convex optimization show randomly initialized gradient descent algorithm or perturbed gradient descent can find a global minimum~\citep{lee2016gradient,ge2015escaping,jin2017escape,du2017gradient}.


==> rank_1.tex <==
In previous sections, we have shown gradient flow automatically balances different layers and this fact implies convergence to global minima in certain problems without any regularization.
In practice, one uses gradient descent with positive step size and the invariance we derived in Section~\ref{sec:conserved} no longer holds.
A natural question is when we use constant positive step, how this discretization affect the invariance we derived in Section~\ref{sec:conserved}.
Unlike gradient flow, in this setting we cannot rely on the differential equations we used for the proof in the previous section and we need detailed study of the gradient descent dynamics.
Furthermore, different problems may require different analysis techniques.


In this section, we initiate the study of gradient descent for learning homogeneous functions. 
We give a detailed analysis of trajectory of gradient descent with constant positive step size for solving rank-$1$ asymmetric matrix factorization problem.
Our main finding is that we can still show the norm of two layers are approximately the same throughout the gradient descent trajectory and this implies \emph{linear} convergence to the global minimum.
Formally we consider the following non-convex minimization problem:
\begin{align*}
\min_{\vect{x} \in \mathbb{R}^{d_1},\vect{y} \in \mathbb{R}^{d_2}} \frac12 \norm{\vect{x}\vect{y}^\top - \mat{M}}_F^2
\end{align*}
where we assume $\mat{M}$ is rank-$1$, i.e., it can be factorized as $\mat{M} = \sigma_1 \vect{u}\vect{v}^\top$ where $\vect{u}$ and $\vect{v}$ are unit vectors and $\sigma_1>0$.
For the ease of presentation we assume $d_1 = \Theta\left(d_2\right)$ and denote $d=\max\left\{d_1,d_2\right\}$.
The gradient descent dynamics for $\vect{x}$ and $\vect{y}$ can be written as
\begin{align*}
\vect{x}_{t+1} &= \vect{x}_t - \eta \left(\vect{x}_t\vect{y}_t^\top - \mat{M}\right)\vect{y}_t \\
\vect{y}_{t+1} &= \vect{y}_t - \eta\left(\vect{y}_t\vect{x}_t^\top - \mat{M}^\top\right)\vect{x}_t.
\end{align*}
Our main theoretical result is the following.
\begin{thm}[Approximately Conserved Quantities and Convergence of GD for Rank-$1$ MF]
\label{thm:rank_1}
Suppose $\vect{x}_0 \sim \cN(0,\delta_1\mat{I})$, $\vect{y}_0 \sim \cN(0,\delta_2 \mat I)$ with $\delta_1 = c_{init} \sqrt{\sigma}_1/\sqrt{d}  $, $\delta_2 =c_{init} \sqrt{\sigma}_1/\sqrt{d}$ for some small constant $0 < c_{init} > \frac{1}{100}$ and $\eta \le \frac{c_{step}}{\sigma_1}$ for some small constant $0 < c_{step} < \frac{1}{10}$.
Then with constant probability over the initialization, for $t=1,\ldots,$ $c_0\le \frac{\abs{\vect{u^\top\vect{x}_t}}}{\abs{\vect{v}^\top \vect{y}_t}}\le C_0$ for some absolute constants $C_0 \ge c_0  > 0$.
Furthermore, after $T = O\left(\frac{1}{\sigma_1\eta}\left(\log d + \log\frac{1}{\epsilon}\right)\right)$ iterations, we have $\norm{\vect{x}_T\vect{y}_T^\top - \mat{M}}_F \le \epsilon \sigma_1$.
\end{thm}
Theorem~\ref{thm:rank_1} shows for $\vect{x}_t$ and $\vect{y}_t$, their strengths in the signal space, i.e. $\abs{\vect{u}^\top \vect{x}_t}$ and $\abs{\vect{v}^\top \vect{y}_t}$ are of the order:  $c_0\le \frac{\abs{\vect{u^\top\vect{x}_t}}}{\abs{\vect{v}^\top \vect{y}_t}}\le C_0$.
This fact can be viewed as a generalization of Corollary~\ref{cor:conserved-F-norm} where here this property only approximately holds.
Since two layer are balanced, we can choose a positive constant step size $\eta \asymp \frac{1}{\sigma_1}$ for all iterations and this leads to linear convergence.
In the following we present our main proof ideas.


\subsection{Proof Sketch of Theorem~\ref{thm:rank_1}}
To analyze the convergence, we define four key quantities.
\begin{align*}
\alpha_t = \vect{u}^\top\vect{x}_t,\quad
\alpha_{t,\perp} = \norm{\vect{u}_\perp^\top\vect{x}_t}_2, \quad
\beta_{t} = \vect{v}^\top \vect{y}_t, \quad
\beta_{t,\perp} = \norm{\vect{v}_\perp^\top \vect{y}_t}_2
\end{align*}
where $\vect{u}_\perp^\top$ and $\vect{v}^\top_{\perp}$ represent the projection matrix onto the complement space of $\vect{u}$ and $\vect{v}$, respectively.
Notice that $\norm{\vect{x}_t}_2^2 = \alpha_t^2 + \alpha_{t,\perp}^2$ and $\norm{\vect{y}_t}_2^2 = \beta_t^2 + \beta_{t,\perp}^2$.
Note if eventually we find a global minimum, we have $\beta_{t,\perp} = 0, \alpha_{t,\perp}=0$ and $\alpha_t \beta_t = \sigma_1$.
It turns out we can write out an explicit formula for the dynamics of the these quantities.
\begin{align*}
\alpha_{t+1} = 
\left(1-\eta\left(\beta_t^2 +\beta_{t,\perp}^2\right)\right)\alpha_t + \eta\sigma_1\beta_t, \quad
&\beta_{t+1} = \left(1-\eta\left(\alpha_t^2+\alpha_{t,\perp}^2\right)\right)\beta_t + \eta_1\sigma_1 \alpha_t\\
\alpha_{t+1,\perp} = \left(1-\eta\left(\beta_t^2+\beta_{t,\perp}^2\right)\right)\alpha_{t,\perp}, \quad
&\beta_{t+1,\perp} = \left(1-\eta\left(\alpha_t^2+\alpha_{t,\perp}^2\right)\right)\beta_{t,\perp}
\end{align*}

Since we use Gaussian initialization, by standard random matrix theory, with overwhelming probability, we know the following facts about these quantities \[
\alpha_0 \asymp \frac{c_{init}\sigma_1}{\sqrt{d}}, \quad \alpha_{0,\perp} \asymp c_{init} \sqrt{\sigma_1}, \quad \beta_0 \asymp\frac{c_{init}\sigma_1}{\sqrt{d}}, \quad\beta_{0,\perp} \asymp c_{init} \sqrt{\sigma_1}.
\]
We also assume signal at the beginning is positive: $\alpha_0 > 0, \beta_0 > 0.$, which holds with probability $0.5$ using Gaussian initialization.


To prove $c_0\le \frac{\abs{\vect{u^\top\vect{x}_t}}}{\abs{\vect{v}^\top \vect{y}_t}}\le C_0$ for all iterations, we cannot only analyze quantity $\frac{\abs{\vect{u^\top\vect{x}_t}}}{\abs{\vect{v}^\top \vect{y}_t}}$ along, the convergence rate to the global minimum also plays an important role in affecting $\frac{\abs{\vect{u^\top\vect{x}_t}}}{\abs{\vect{v}^\top \vect{y}_t}}$.
We divide the dynamics into two stages.
\begin{thm}[Stage 1: Escaping from $(\vect{
0},\vect{0})$ Saddle Point]\label{thm:rank_1_stage_1}
Let $T := \argmin_{t} \left\{\alpha_t^2 + \beta_t^2 \le c_1\sigma_1\right\}$ for $c_1 = 1/2$.
If $\eta \le \frac{c_{step}}{\sigma_1}$, then for $t=1,\ldots,T-1$, the followings hold\begin{itemize}
\item Magnitude in complement space remain small: $\xi_t \le \xi_0$;
\item Growth of magnitude in signal space: $\abs{\alpha_{t+1}+\beta_{t+1}} \ge \left(1+\frac{\eta\sigma_1}{3}\right) \abs{\alpha_t+\beta_t}$;
\item Bounded ratio between two layers: $\abs{\alpha_t - \beta_t} \le c_{diff}\abs{\alpha_t+\beta_t}$ where $c_{diff} \triangleq \frac{\abs{\alpha_0-\beta_0}}{\abs{\alpha_0+\beta_0}}$.
\end{itemize}
Furthermore, after at most $T_1 = O\left(\frac{1}{\eta\sigma_1}\log\left(\frac{\sigma_1}{\alpha_0+\beta_0}\right)\right)$ iterations, $T_1 \le T$, we have $\alpha_{T_1} \beta_{T_1} \ge c \sigma_1$ for some small constant $0 < c < 1$.
\end{thm}
In this stage, the strength in the noise space remains small ($\xi_t \le \xi_0$) and the strength in the signal space is growing ($\abs{\alpha_{t+1}+\beta_{t+1}} \ge \left(1+\frac{\eta\sigma_1}{3}\right) \abs{\alpha_t+\beta_t}$).
Further, because  $\abs{\alpha_t - \beta_t} \le c_{diff}\abs{\alpha_t+\beta_t}$, we know $\frac{1-c_{diff}}{1+c_{diff}}\le \frac{\alpha_t}{\beta_t} \le \frac{1+c_{diff}}{1-c_{diff}}$, which is our desired result.
Here we consider $\abs{\alpha_t - \beta_t} / \abs{\alpha_t - \beta_t}$ instead of directly bounding $\frac{\alpha_t}{\beta_t}$ because the dynamics of $\abs{\alpha_t - \beta_t} / \abs{\alpha_t - \beta_t}$ is much simpler to analyze.
This will be apparent in the proof.


Now we enter stage 2, which is essentially a local convergence phase.
The following theorem characterizes the behaviors of the strength in the signal and in the noise space in this stage.
\begin{thm}[Stage 2: Local Convergence]\label{thm:rank_1_stage_2}

Suppose at $T_1$-th iteration, the followings hold \begin{align*}
\alpha_{T_1}\beta_{T_1} \ge c\sigma_1, \quad
\alpha_{T_1,\perp}^2+\beta_{T_1,\perp}^2 \le &10c_{init} \sigma_1,\quad
\abs{\alpha_{T_1}-\beta_{T_1}} \le c_{diff}\abs{\alpha_{T_1}+\beta_{T_1}}
\end{align*} where $c > 1/5$, $c_{init} < 1/100$, $c_{diff}< 1$ and $\eta \le \frac{c_{step}}{\sigma_1}$ for $c_{step} \le 1/100$.
Let $\tau_t = \min\{\alpha_t,\beta_t\}$ and $\tau_{min}  \triangleq \frac{\tau_{T_1}}{2}$.
Then for all $t = T+1,T+2,\ldots$, the followings hold 
\begin{align*}
\tau_t \ge \prod_{i=T+1}^{t}\left(1-\eta\xi_0\left(1-\eta\tau_{min}^2\right)^{i-T}\right)\tau_T, \quad
\xi_t \le \left(1-\eta\tau_{min}^2\right)^{t-T} \xi_0, \quad \alpha_t\beta_t \le \sigma_1.
\end{align*}
\end{thm}
In Theorem~\ref{thm:rank_1_stage_2}, $\tau_t$ characterizes the smaller signal strength in $\vect{x}_t$ and $\vect{y}_t$ and $\xi_t$ characterizes the strength in the noise space.
Note even though $\tau_t$ may decrease, with some algebra, Theorem~\ref{thm:rank_1_stage_2} shows $\tau_t$ is uniformly bounded by $\Omega\left(\sqrt{\sigma_1}\right)$ for all $t \ge T_1$. 
Combining with the fact that $\alpha_t\beta_t \le \sigma_1$, we know $c_0\le \frac{\alpha_t}{\beta_t} \le C_0$ for all $t \ge T_1$.
Similar to Theorem~\ref{thm:rank_1_stage_1}, here we consider $\tau_t$ and $\alpha_t\beta_t$ instead of directly analyzing $\frac{\alpha_t}{\beta_t}$ because dynamics of $\tau_t$ and $\alpha_t\beta_t$ are easier to analyze.

A directly corollary is the following local convergence rate result, which is proved by examining the dynamics of $\alpha_t\beta_t$.
\begin{cor}\label{cor:rank_1local_convergence_rate}
Under the same assumptions as in Theorem~\ref{thm:rank_1_stage_2}, we have after $T_2 = O\left(\frac{1}{\eta \sigma_1}\log\left(\frac{1}{\epsilon}\right)\right)$ iterations, $
\norm{\vect{x}\vect{y}^\top - \mat{M}}_F^2 \le \epsilon^2 \sigma_1^2.$
\end{cor}
Theorem~\ref{thm:rank_1_stage_1}, Theorem~\ref{thm:rank_1_stage_2} and Corollary~\ref{cor:rank_1local_convergence_rate} together imply Theorem~\ref{thm:rank_1}.




















  
